CoMatch: Semi-supervised Learning with Contrastive Graph Regularization

Semi-supervised learning has been an effective paradigm for leveraging unlabeled data to reduce the reliance on labeled data. We propose CoMatch, a new semi-supervised learning method that unifies dominant approaches and addresses their limitations. CoMatch jointly learns two representations of the training data, their class probabilities and low-dimensional embeddings. The two representations interact with each other to jointly evolve. The embeddings impose a smoothness constraint on the class probabilities to improve the pseudo-labels, whereas the pseudo-labels regularize the structure of the embeddings through graph-based contrastive learning. CoMatch achieves state-of-the-art performance on multiple datasets. It achieves substantial accuracy improvements on the label-scarce CIFAR-10 and STL-10. On ImageNet with 1% labels, CoMatch achieves a top-1 accuracy of 66.0%, outperforming FixMatch by 12.6%. Furthermore, CoMatch achieves better representation learning performance on downstream tasks, outperforming both supervised learning and self-supervised learning. Code and pre-trained models are available at https://github.com/salesforce/CoMatch.

==> table/augmentation.tex <==



==> table/transfer.tex <==
\begin{table*}[!t]
%\small
	\centering
	\begin{tabular}	{l l | c  c | c  c  }
	\toprule
    \multirow{2}{*}{Method} &  \multirow{2}{*}{\#Epochs} & \multicolumn{2}{c|}{Linear classification} &  \multicolumn{2}{c}{Object detection} \\
	 & & Places205 & VOC07 & VOC07+12 & COCO \\
	\midrule
	Supervised & 90 & 53.2& 87.5& 81.3&\\
	MoCo v2~\cite{mocov2} &800 & 52.9& 86.8 & 82.5 &\\
	SwAV~\cite{swav} &400 & &86.9 & &\\		
	CoMatch-M (1\%)&400 & 53.5&87.7 & &\\
	\hline
	SwAV (multi-crop)~\cite{swav} &800 & 56.7&88.9 &82.6 &\\	
	\bottomrule
	\end{tabular}	
	\caption
		{\small	
		Accuracy .
		}
	\label{tbl:transfer}
\end{table*}		
